Privacy-Protecting Techniques for Behavioral Biometric Data: A Survey

Our behavior (the way we talk, walk, act or think) is unique and can be used as a biometric trait. It also correlates with sensitive attributes like emotions and health conditions. Hence, techniques to protect individuals privacy against unwanted inferences are required, if such data is planned to be processed. To consolidate knowledge in this area, we systematically review applicable anonymization techniques. We taxonomize and compare existing solutions regarding privacy goals, conceptual operation, advantages, and limitations. We review anonymization techniques for the behavioral biometric traits of voice, gait, hand motions, eye-gaze, heartbeat (ECG), and brain activity (EEG). Our analysis shows that some behavioral traits (e.g., voice) have received much attention, while others (e.g., eye-gaze, brain activity) are mostly neglected. We also find that the evaluation methodology of behavioral anonymization techniques can be further improved.

==> sections/dataset_table.tex <==
\begin{table*}[!ht]
\begin{center}
\begin{tabularx}{0.95\textwidth}{|p{4cm}|X|X|X|X|}
\hline
Name & Participants & Published & Source & Trait \\
\hline
TIMIT & 630 & 1993  & \cite{TIMIT} & Voice\\
Albayzin & 164 & 1993 & \cite{albayzin} & Voice\\
YOHO & 137 & 1994 & \cite{YOHO} & Voice\\
BioSecureID & 400 & 2009 & \cite{BioSecureID} & Voice\\
Billeb et al. & 701 & 2014 & \cite{billeb_biometric_2015} & Voice \\
Librispeech & 1166 & 2015 & \cite{Librispeech}& Voice \\
RSR2015 & 300 & 2015  & \cite{RSR2015}& Voice\\
VoxCeleb & 1251 & 2018  & \cite{VoxCeleb} & Voice\\
CSTR VCTK Corpus & 110 & 2019 & \cite{vctk} &  Voice \\
VCC 2016 & 10 & 2016 & \cite{vcc2016} & Voice \\
\hline
CASIA-B  & 124 & 2005 & \cite{szhengICIP2011} & Gait\\
%%i3DPost & 8 & 2009  & \cite{gkalelis2009i3dpost} & Gait\\
BEHAVE & 125 & 2010 & \cite{blunsden2010behave} & Gait\\
OU-ISIR  & 200 & 2012 & \cite{Makihara_CVATN2012} & Gait\\
EPIC-Kitchens & 32 & 2020 & \cite{Damen2020Collection} & Gait\\
IITMD-WFP & 31 & 2021 & \cite{thapar_anonymizing_2021} & Gait\\
\hline
MCYT baseline corpus  & 330 & 2003 & \cite{ortega-garcia_mcyt_2003} & Hand motion\\
%SVC2004 & 100 & 2004 & \cite{kanade_svc2004_2004} & Hand motion \\
%GREYC  & 133 & 2009 & \cite{giot_greyc_2009} & Hand motion\\
%MNIST  & 500 & 2012 & \cite{li_deng_mnist_2012} & Hand motion\\
%Web-based keystroke  & 83 & 2012 & \cite{giot_web-based_2012} & Hand motion\\
%SMILE & 30 & 2018 & \cite{SMILE} & Hand motion\\
%ASLLRP & 33 & 2022 & \cite{ALSVideo}  & Hand motion\\ 
\hline
DGaze & 22 & 2020 & \cite{isha2020iros} & Eye-Gaze\\
%%ET-DK2 & 18 & 2021 & \cite{brendan_david_john_2021_4642612} & Eye-Gaze\\
%VR-Saliency & 169 & 2018 & \cite{8269807} & Eye-Gaze\\
%Gaze Prediction & 43 & 2018 & \cite{8578657} & Eye-Gaze\\
%Video viewing & 50 & 2017 & \cite{VideoViewing} & Eye-Gaze\\
%MPIIDPEye & 20 & 2019 & \cite{steil19_etra_2} & Eye-Gaze\\
%OpenEDS & 157 & 2019 & \cite{OpenEDS} & Eye-Gaze\\
%EHTask & 30 & 2022 & \cite{hu22_EHTask} & Eye-Gaze\\
%DOVES & 29 & 2009 & \cite{doves} & Eye-Gaze\\
\hline
%SUNY EEG database  & 50 & 1999 & \cite{EEGDatabase} & Brain activity\\
%UCI EEG database & 122 & 1999 & \cite{UCIEEG} & Brain activity\\
%DEAP & 32 & 2011 & \cite{5871728} & Brain activity\\
%DREAMER & 23 & 2018 & \cite{katsigiannis_stamos_2017_546113} & Brain activity\\
%SEED & 15 & 2015 & \cite{zheng2015investigating} & Brain activity\\
\hline
MIT-BIH ECG Arrhythmia & 47 & 1979 & \cite{MIT-DB} & Heartbeat\\
%%MIT-BIH Noise Stress Test & 2 & 1984 & \cite{MIT-SN} & Heartbeat\\
%Physikalisch Technische Bundesanstalt & 290 & 1995 & \cite{PTB-DB} & Heartbeat\\
\hline
\end{tabularx}
\end{center}
\caption{An overview of used behavioral biometric datasets.}\label{table:datasets}
\end{table*}

==> sections/foobar.tex <==
\begin{table*}[!ht]
\begin{center}
\begin{tabularx}{0.95\textwidth}{|p{4cm}|X|X|X|X|}
\hline
Name & Participants & Published & Source & Trait \\
\hline
TIMIT & 630 & 1993  & \cite{TIMIT} & Voice\\
Albayzin & 164 & 1993 & \cite{albayzin} & Voice\\
YOHO & 137 & 1994 & \cite{YOHO} & Voice\\
BioSecureID & 400 & 2009 & \cite{BioSecureID} & Voice\\
Billeb et al. & 701 & 2014 & \cite{billeb_biometric_2015} & Voice \\
Librispeech & 1166 & 2015 & \cite{Librispeech}& Voice \\
RSR2015 & 300 & 2015  & \cite{RSR2015}& Voice\\
VoxCeleb & 1251 & 2018  & \cite{VoxCeleb} & Voice\\
CSTR VCTK Corpus & 110 & 2019 & \cite{vctk} &  Voice \\
VCC 2016 & 10 & 2016 & \cite{vcc2016} & Voice \\
\hline
CASIA-B  & 124 & 2005 & \cite{szhengICIP2011} & Gait\\
%%i3DPost & 8 & 2009  & \cite{gkalelis2009i3dpost} & Gait\\
BEHAVE & 125 & 2010 & \cite{blunsden2010behave} & Gait\\
OU-ISIR  & 200 & 2012 & \cite{Makihara_CVATN2012} & Gait\\
EPIC-Kitchens & 32 & 2020 & \cite{Damen2020Collection} & Gait\\
IITMD-WFP & 31 & 2021 & \cite{thapar_anonymizing_2021} & Gait\\
\hline
MCYT baseline corpus  & 330 & 2003 & \cite{ortega-garcia_mcyt_2003} & Hand motion\\
%SVC2004 & 100 & 2004 & \cite{kanade_svc2004_2004} & Hand motion \\
%GREYC  & 133 & 2009 & \cite{giot_greyc_2009} & Hand motion\\
%MNIST  & 500 & 2012 & \cite{li_deng_mnist_2012} & Hand motion\\
%Web-based keystroke  & 83 & 2012 & \cite{giot_web-based_2012} & Hand motion\\
%SMILE & 30 & 2018 & \cite{SMILE} & Hand motion\\
%ASLLRP & 33 & 2022 & \cite{ALSVideo}  & Hand motion\\ 
\hline
DGaze & 22 & 2020 & \cite{isha2020iros} & Eye-Gaze\\
%%ET-DK2 & 18 & 2021 & \cite{brendan_david_john_2021_4642612} & Eye-Gaze\\
%VR-Saliency & 169 & 2018 & \cite{8269807} & Eye-Gaze\\
%Gaze Prediction & 43 & 2018 & \cite{8578657} & Eye-Gaze\\
%Video viewing & 50 & 2017 & \cite{VideoViewing} & Eye-Gaze\\
%MPIIDPEye & 20 & 2019 & \cite{steil19_etra_2} & Eye-Gaze\\
%OpenEDS & 157 & 2019 & \cite{OpenEDS} & Eye-Gaze\\
%EHTask & 30 & 2022 & \cite{hu22_EHTask} & Eye-Gaze\\
%DOVES & 29 & 2009 & \cite{doves} & Eye-Gaze\\
\hline
%SUNY EEG database  & 50 & 1999 & \cite{EEGDatabase} & Brain activity\\
%UCI EEG database & 122 & 1999 & \cite{UCIEEG} & Brain activity\\
%DEAP & 32 & 2011 & \cite{5871728} & Brain activity\\
%DREAMER & 23 & 2018 & \cite{katsigiannis_stamos_2017_546113} & Brain activity\\
%SEED & 15 & 2015 & \cite{zheng2015investigating} & Brain activity\\
\hline
MIT-BIH ECG Arrhythmia & 47 & 1979 & \cite{MIT-DB} & Heartbeat\\
%%MIT-BIH Noise Stress Test & 2 & 1984 & \cite{MIT-SN} & Heartbeat\\
%Physikalisch Technische Bundesanstalt & 290 & 1995 & \cite{PTB-DB} & Heartbeat\\
\hline
\end{tabularx}
\end{center}
\caption{An overview of used behavioral biometric datasets.}\label{table:datasets}
\end{table*}
